Summaries as Captions: Generating Figure Captions for Scientific Documents with Automated Text Summarization

Good figure captions help paper readers understand complex scientific figures. Unfortunately, even published papers often have poorly written captions. Automatic caption generation could aid paper writers by providing good starting captions that can be refined for better quality. Prior work often treated figure caption generation as a vision-to-language task. In this paper, we show that it can be more effectively tackled as a text summarization task in scientific documents. We fine-tuned PEGASUS, a pre-trained abstractive summarization model, to specifically summarize figure-referencing paragraphs (e.g., "Figure 3 shows...") into figure captions. Experiments on large-scale arXiv figures show that our method outperforms prior vision methods in both automatic and human evaluations. We further conducted an in-depth investigation focused on two key challenges: (i) the common presence of low-quality author-written captions and (ii) the lack of clear standards for good captions. Our code and data are available at: https://github.com/Crowd-AI-Lab/Generating-Figure-Captions-as-a-Text-Summarization-Task.

==> sections/limitation.tex <==
\begin{itemize}
    \item Our method needs mentions to produce captions, but identifying the mentions for figures in real-world data is not always easy. 18.81\% of figures in original \oldDataset did not have any identified mentions, which we excluded in this work.
Many factors contributed to the gap, including
errors caused by upstream components such as image extraction or image type classification (\eg, table),
unexpected figure index formats (\eg, ``Figure VIII'', ``Figure C·1'',``Fig.Fig. 4(b)''),
PDF parsing errors, or 
the figure never being explicitly referred to in the paper. Our procedure is not applicable to such cases.

\item
Our paper focused on non-compound line charts in arXiv papers, and the human evaluation only focused on NLP papers.
More research is needed to examine the generalizability.

\item 
The proposed method uses texts instead of images as the primary information source, so it is not capable of capturing the visual content that only occurs in the image.

\item 
The quality of the generated caption in our approach is bounded by the text quality of the paragraph.
When the article is poorly written, our models will likely struggle.

\end{itemize}

==> tables/text-matching-table.tex <==
\begin{table}[t]
\tiny
% \scriptsize
\small
\centering
\addtolength{\tabcolsep}{-0.12cm}

\begin{tabular}{ll  rrrr  rr}
\toprule
% \hline
\textbf{} & \textbf{} & \multicolumn{4}{c}{\textbf{Words from}} & \multicolumn{2}{c}{\textbf{Baseline}} \\ 
\cmidrule(lr){3-6}
\cmidrule(lr){7-8}
% \hline
 &  & \multicolumn{1}{c}{\textbf{OCR}} & \multicolumn{1}{c}{\textbf{Whole Caption}} & \multicolumn{1}{c}{\textbf{1st Caption}} & \multicolumn{1}{c}{\textbf{M Mentions (M}$\mathbf{\geq}$\textbf{1)}} & \multicolumn{1}{c}{\textbf{NON-mention S}} & \multicolumn{1}{c}{\textbf{random S}} \\ 
 \midrule

\multirow{5}{*}{\shortstack{\textbf{Words}\\\textbf{occur}}} & \textbf{OCR} & 100.00 & 8.26 & 6.66 & 7.78 & 5.39 & 0.47 \\ 
\cmidrule{2-8}
% \cline{2-8} 
 & \textbf{Whole Caption} & 8.11 & 100.00 & 62.37 & 27.20 & 19.76 & 0.16 \\ 
 \cmidrule{2-8}
%  \cline{2-8} 
 & \textbf{1st Caption} & 5.07 & 54.78 & 100.00 & 19.16 & 12.81 & 0.01 \\ 
 \cmidrule{2-8}
%  \cline{2-8} 
 & \textbf{M Mentions (M}$\mathbf{\geq}$\textbf{1)} & 7.74 & 27.29 & 22.99 & 100.00 & 24.49 & 0.26 \\ 
 \midrule
%  \hline
\multirow{2}{*}{\textbf{Baseline}} & \textbf{NON-mention S} & 5.32 & 19.77 & 14.88 & 24.46 & 100.00 & 0.21 \\ 
\cmidrule{2-8} 
 & \textbf{random S} & 1.65 & 0.93 & 0.64 & 1.22 & 1.11 & 100.00 \\  
%  \hline
\bottomrule
\end{tabular}
\addtolength{\tabcolsep}{+0.12cm}

\caption{Text matching between image texts, captions and mentions of each figure.}
\label{tab:analysis_ocr-caption-mention}

\end{table}
